Learning to Explain: A Model-Agnostic Framework for Explaining Black Box Models

We present Learning to Explain (LTX), a model-agnostic framework designed for providing post-hoc explanations for vision models. The LTX framework introduces an "explainer" model that generates explanation maps, highlighting the crucial regions that justify the predictions made by the model being explained. To train the explainer, we employ a two-stage process consisting of initial pretraining followed by per-instance finetuning. During both stages of training, we utilize a unique configuration where we compare the explained model's prediction for a masked input with its original prediction for the unmasked input. This approach enables the use of a novel counterfactual objective, which aims to anticipate the model's output using masked versions of the input image. Importantly, the LTX framework is not restricted to a specific model architecture and can provide explanations for both Transformer-based and convolutional models. Through our evaluations, we demonstrate that LTX significantly outperforms the current state-of-the-art in explainability across various metrics.

==> latex/02_related.tex <==




While the task of explaining ViTs is relatively new, many earlier works have been focused on explaining CNNs. The two most dominant approaches are based on computing gradients w.r.t. the input or internal activation maps~\cite{sundararajan2017axiomatic,selvaraju2017grad,chattopadhay2018grad,barkan2021gam,jiang2021layercam,barkan2023dix,barkan2023six,Barkan_2023_ICCV},
and attribution methods~\cite{montavon2017explaining,shrikumar2017learning,nam2020relative}.
Most relevant to this work, however, is a line of work in which a learning model is employed in order to produce explanations for the explained model. %
For example, in~\cite{chen2018learning}, a theoretical framework for instance-wise feature selection was presented for per-instance explanations. 
Another work by~\cite{fong2017interpretable} proposed extracting explanations by training a model to identify the image parts most influential in a classifier's decision. %













There are relatively fewer works focusing on explaining Vision Transformers (ViTs). Early attempts primarily involved leveraging attention scores. However, the aggregation of attention scores from different layers poses an ongoing research challenge. For instance, simple averaging has been observed to induce blurring, and researchers have explored various heuristics to address this issue~\cite{abnar2020quantifying}.%
Transformer Attribution (T-Attr)~\cite{chefer2021transformer} %
assigns local relevance based on a Deep Taylor Decomposition (DTD) and propagates it forward through the layers. Their approach accounts for skip-connections which have challenged previous methods. 
The authors later generalized this method and presented Generic Attention Explainability (GAE) for explaining Bi-Modal transformers~\cite{chefer2021generic}. %













==> latex/sanity.tex <==
In order to further evaluate validity of EEA as an explanation method, we conducted both the \emph{parameter randomization} and \emph{data randomization} sanity tests suggested
by~\cite{adebayo2018sanity}. %

\subsubsection{Parameter Randomization Test}
\label{subsec:paramrand_test}
The parameter randomization test involves a comparison of the explanation maps generated by an explanation method using two distinct configurations: (1) a ``normal'' setup where the explained model is an optimized model. %
and (2) a random setup, in which the same explained model is used but with random weights, i.e., a ViT classification model initialized with random attention weights. For explanation methods that depend on the specific characteristics of the explained model, substantial disparities are expected between the explanation maps produced for the trained model and those generated for the random model. Conversely, if the explanation maps exhibit similarity, it indicates that the explanation method is insensitive to the model being explained, suggesting limited explainability power. %

Given a trained ViT-B model, we perform randomization of the model's weights, starting from the top layer and successively moving down to the bottom layer. This process leads to the destruction of the learned weights from the top to the bottom layers.
 Figure~\ref{fig:sanity_checkes_metric_cascade} presents the Spearman correlation (averaged on 50K samples) between the original explanation map obtained by EEA on a trained ViT-B %
 and the explanation map obtained by EEA for a ViT-B with cascade randomization. %
 ViT-B model uses 12 layers of attention. The markers on the x-axis are between '1' and '13' (total of 12 layers) where $x=k$ means that the weights of the last $k$ layers of the model were randomized. At $x=1$ there is no randomization, hence the correlation with the original model is perfect. Starting from $x=2$ and up to $x=13$, the graph depicts a progressive cascade randomization of the original model. We observe that as more layers are randomized, the correlation with the explanation map of the original model significantly deteriorates. This behavior showcases the sensitivity of EEA to the model's parameters - a desired trait for any explanation method~\cite{adebayo2018sanity}. In our GitHub repository, we further provide an additional version of this sanity test in which a layer-by-layer randomization is employed (one layer at a time), and qualitative examples demonstrating the effect of randomization on the explanation maps.





\begin{figure}[t]
    \centering
    \includegraphics[scale=0.55]{figures/cascading_random.png}\vspace{-3mm}
    \caption{\textbf{Parameter Randomization}: 
    A ViT-B model which was trained on the ImageNet dataset is subjected to a cascading weight randomization beginning from the last layer backward. The graph depicts the Spearman rank correlation (averaged on 50K examples) between the explanation produced by EEA using the original and the randomized models. %
    }
    \label{fig:sanity_checkes_metric_cascade}
    \vspace{-5mm}
\end{figure}














\subsubsection{Data Randomization Test}
\label{subsec:datarand_test}
The data randomization test is a statistical method used to test the sensitivity of the explanation method to the labeling of the data which was used by the explained model.
For this test, we produced two explanation maps using an identical architecture but with two different datasets: one with the original labels and another with randomly permuted labels. A desired result is that the explanation method produces explanation maps that differ significantly between the two cases.
However, if the method is insensitive to the permuted labels, it indicates that it does not depend on the relationship between instances and labels that exists in the original data. 
To conduct the data randomization test, we permute the training labels in the dataset and train a ViT classification model to achieve a training set accuracy greater than 95\%. Note that the resulting model's test accuracy is never better than randomly guessing a label. We then compute explanations on the same test inputs for both the model trained on the true labels and the model trained on the randomly permuted labels.  

Figure~\ref{fig:sanity_checkes_visual_bxplt}  presents a box plot computed for the Spearman correlation values obtained for paired explanation maps (50K examples): one produced using the original model, and the other produced by the model trained with the permuted labels. As we can see,  the average correlation values are very low indicating EEA's sensitivity to the labeling of the dataset. Hence, we conclude that EEA successfully passes the data randomization test. In our GitHub repository, we further provide qualitative results demonstrating the sensitivity of EEA to data randomization.


\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{figures/spear_corr.pdf}
    \vspace{-5mm}\caption{\textbf{Data Randomization Test}: Spearman rank correlation box plot for EEA with a ViT-B model.} %
    \label{fig:sanity_checkes_visual_bxplt}
    \vspace{-3mm}
\end{figure}





